Evading Malware Analysis Using Reverse Execution

Malware is a security threat, and various means are adapted to detect and block them. In this paper, we demonstrate a method where malware can evade malware analysis. The method is based on single-step reverse execution of code using the self-debugging feature. We discuss how self-debugging code works and use that to derive reverse execution for any payload. Further, we demonstrate the feasibility of a detection evading malware through a real implementation that targets Linux x86-64 architecture for a reference implementation. The reference implementation produces one result when run in one direction and a different result when run in the reverse direction.

==> Links.tex <==
Links
-----

1. http://www.articleworld.org/index.php?title=1260_(computer_virus)&printable=yes
2. https://en.wikipedia.org/wiki/Dark_Avenger#Viruses
3. http://virus.wikidot.com/marburg
4. https://www.f-secure.com/v-descs/marburg.shtml
5. https://malwiki.org/index.php?title=Gollum
6. https://malwiki.org/index.php?title=CTX
7. https://malwiki.org/index.php?title=Dengue

==> methodology.tex <==
We can describe how the method works here

==> rel_work.tex <==
The existing Internet ecosystem addresses the problem of masking host identity in many ways. The VPN-based solutions providing end-to-end encryption at the network layer (using IPSec \cite{rfc4301}) serve the purpose directly. However, VPN-based solutions are a threat to network performance \cite{vpn_bottleneck}. The authors in \cite{tor} propose a method of domain fronting in which the fronting server establishes a secure connection with the client using its server name. Later this connection is extended to the intended content server by establishing another HTTPS tunnel within an already established HTTPS tunnel. The major drawback of this method is the increased workload of double encryption. The recently developed transport protocol Quick UDP Internet Connections (QUIC) \cite{quic} provides the in-built support for masking host identity through obfuscated SNI. It uses an `initial secret' along with the pre-defined SHA Hash algorithms \cite{hash_survey} to obfuscate the initial TLS handshake message along with SNI. It does not provide confidentiality but ensures that SNI is not directly readable by network middle-boxes. QUIC is a relatively new protocol and a very small section of Internet services compared to the TCP-TLS combination use it. So in this work, we focus on masking host identity through encrypting SNI in TLS handshake. 

The attempt to encrypt/decrypt SSL/TLS handshake parameter is done in \cite{csk_ssl}. It proposes the Combined Symmetric Key (CSK) based SSL handshake that uses CSK technology to authenticate both communication sides and uses the symmetric key to encrypt and decrypt secret information, i.e., server authentication code. The overhead associated with this scheme for adding one more level of authentication makes it less suitable to mask the host identity. 

A standardization body acknowledges the need for encrypted SNI (E-SNI) with the related issues and requirements well documented in the internet-draft \cite{draft-ietf-tls-sni-encryption-09}. It categorizes various E-SNI requirements as attack prevention, fronting server-related, and other security considerations. The E-SNI is still not available as an Internet standard, but the internet-draft in an experimental version is available \cite{draft-ietf-tls-esni-13} that proposes to encrypt the entire ``clientHello" message. A slightly different version of it is already implemented and commercialized by ``Cloudflare" \cite{cf_esni} that encrypts only the SNI portion of the ``clientHello" message. It uses the Diffie-Hellman key exchange algorithm to generate a shared encryption key over an untrusted channel. This method's main drawback is that it requires a considerable amount of pre-handshake processing and requires the client and server to exchange the public portion of the generated symmetric key to encrypt and decrypt SNI. This requirement raises the security issues that need mitigation using persistent security credential modifications.  

Thus, previous works suffer from various challenges in masking host identity, such as network performance and added security concerns. Our SNI encryption method does not suffer from these limitations as it encrypts the SNI using existing secure channel methods and does not add significant overhead. It not only hides SNI from middle-boxes but also hides the plain-text server certificate, if any. Thus, it makes the entire SSL/TLS handshake in question transparent to network middle-boxes without adding any extra layer of encryption.

==> self-healing.tex <==
A self-healing code is a program which has ability to restore itself into original state, once it is determined that running code has been altered. This is useful from malware developer's point of view as binary patching is a common practice during malware analysis. Patching is generally used to disable features like anti-debugging, VM detection, sandbox detection etc.

\noindent
\textbf{Detecting patching:}
To detect patching, it is generally bad idea to directly match bytes in executable code with known good copy stored elsewhere, as this becomes very easy to circumvent (analyst can alter stored good copy as well). A better method is to calculate some checksum of code, then perform checks on calculated checksum.A reference implementation using CRC is given below:

\begin{lstlisting}[frame=single]
std::array<std::uint_fast32_t, 256> 
    generate_crc_lookup_table() noexcept
{
    auto const reversed_polynomial = 
        std::uint_fast32_t{0xEDB88320uL};

    struct byte_checksum
    {
        std::uint_fast32_t operator()() 
                noexcept
        {
            auto checksum = 
                static_cast<
                std::uint_fast32_t>(n++);

            for (auto i = 0; i < 8; ++i)
                checksum = 
                (checksum >> 1) ^ 
                ((checksum & 0x1u) ?
                reversed_polynomial : 
                0);

            return checksum;
        }

        unsigned n = 0;
    };

    auto table = 
    std::array<std::uint_fast32_t, 256>{};
    std::generate(table.begin(), 
                  table.end(), 
                  byte_checksum{});

    return table;
}

template <typename InputIterator>
std::uint_fast32_t crc(
    InputIterator first, 
    InputIterator last)
{
    static auto const table = 
        generate_crc_lookup_table();

    return 
        std::uint_fast32_t{0xFFFFFFFFuL} &
        ~std::accumulate(first, last,
        ~std::uint_fast32_t{0} & 
        std::uint_fast32_t{0xFFFFFFFFuL},
        [](std::uint_fast32_t checksum, 
            std::uint_fast8_t value)
            { return table[(checksum
                ^ value) & 0xFFu]
                ^ (checksum >> 8); });
}

bool isFunctionPatched
(const unsigned char *func, 
const size_t& machine_code_size, 
const std::uint32_t& checksum)
{
    bool result = true;

    std::vector<unsigned char> 
        machine_code;

    for (auto i = 0; 
            i < machine_code_size; 
            ++i)
    {
        machine_code.push_back(*(func+i));
    }

    uint32_t value = 
        crc(machine_code.begin(), 
        machine_code.end());

    result = (value != checksum);
    return result;
}
\end{lstlisting}

Although we are simply comparing the calculated checksum with known good checksum, a good design will use the calculated checksum for indirect verification. Using checksum for decryption key for certain part of code, or using it as an offset to resolve some symbols in code are some of the common strategies for indirect verification.

\textbf{Unpatching the code:}
Unpatching the code is a bit trickier to get right, as we need to have multiple copies of original code, while still ensuring that backup copies (i.e. the copies which are used to restore the original code) cannot be compromised easily.
Since security of backup copies of code is out of scope of this paper, we are going to limit ourselves to only unpatching part of the code. At very basic level, it works as follows:
\begin{enumerate}
\item Find the page size at given platform
\item Find the pages where recovery is to be performed
\item Optional: take backup of existing memory protections on target pages
\item Change memory permissions on target pages to allow read/write
\item Overwrite the pages with original code
\item Either restore permissions from step 3, otherwise add permission for execute.
\end{enumerate}

A reference implementation for the above will look something like this:

\begin{lstlisting}[frame=single]
bool unpatchFunction
    (unsigned char *func, 
    const std::vector<unsigned char>& 
    machine_code)
{
    bool result = false;

    long pagesize = sysconf(_SC_PAGESIZE);
    unsigned long page_start = 
        (unsigned long)func & 
        ~(pagesize - 1);

    if (mprotect(
            (void*)page_start, 
            pagesize, 
                PROT_READ | 
                PROT_WRITE | 
                PROT_EXEC
            ) != 0)
    {
        return false;
    }

    for (auto i = 0; 
        i < machine_code.size(); 
        ++i)
    {
        if (*(func + i) != 
                machine_code[i]) {
            *(func + i) = machine_code[i];
            result = true;
        }
    }

    return result;
}
\end{lstlisting}
